Representations for Question Answering from Documents with Tables and Text

Tables in Web documents are pervasive and can be directly used to answer many of the queries searched on the Web, motivating their integration in question answering. Very often information presented in tables is succinct and hard to interpret with standard language representations. On the other hand, tables often appear within textual context, such as an article describing the table. Using the information from an article as additional context can potentially enrich table representations. In this work we aim to improve question answering from tables by refining table representations based on information from surrounding text. We also present an effective method to combine text and table-based predictions for question answering from full documents, obtaining significant improvements on the Natural Questions dataset.

==> analysis.tex <==
\section{Analysis}

\subsection{Which Context Matters the Most?}
In our analysis we are interested to look at what exactly from the context helps the model most. In order to do this analysis, we look at the difference the context attention makes to the predictions when present across a few parameters. More specifically, we compare the outputs (scores) of our best context-aware system with outputs extracted using the same system but disabled context attention. Because only 12\% of the table entries have corresponding context matching, we assume that during training the system was capable to handle ``no-match" scenario pretty well. In our analysis, we compare the scores produced by the regular context-aware system with the scores produced by the same system but with simulated ``no match for any entries" scenario. This allows us to look at the differences of the scores, and better understand instances where the system takes into account text context. 

First, we look at how much does the model is capable to infer the information about the high-probability answer from the the context. Since for our context representation embeddings we take a system that was finetuned on the whole NQ dataset, our intuition was that information about high 

We found that the score increased in 95\% of the cases when the corresponding text-based match had a high probability ($>0.5$)  of being a correct answer (described by a start or an end of the span). On an average in those cases the score increased by $0.33 (\pm 0.34)$ points (mean(std)). In comparison, the average score difference for all the matches is $-0.02 (\pm 0.07)$. One the other side, only 38\% of all QA pairs in NQTables subset have a table-text match for the tokens in the correct answer span. Those result suggest that the system indeed is capable of inferring information about the probable answers from the text-based model. Similarly, we look which one of the unigram/bigram/trigram matches result in a higher score change. This is done by calculating the mean of a change in score for each type of n-grams, resulting the change in scores of $-0.026, -0.020, -0.014$ for 1-, 2-, and 3-grams correspondingly. Those results suggest that trigram matches affect model the most. Similarly, we look at the number of corresponding matches found in the surrounding article. The plot of mean score change as a function of number of matches in the article is shown in Figure \ref{fig: num_matches}. Those numbers suggest that single match in a text has a greater affect on the corresponding table entry.
%[1:-0.00133, 2:-0.01174, 3:-0.01902, 4:-0.03045, 6:-0.04596, 12:-0.09962]






==> intro.tex <==
\section{Question Answering on Tables}
Tables are a common type of information representation used all across Internet. With an average of 3.5 billion Google search queries a day, question answering on tables is an important task that translates into thousands of search queries every second about information present in tables. In general, research on Question Answering (QA) can be categorized in terms of the resources that are used in answering the question: text documents (often referred as \textit{unstructured} text in the literature), tables, or a structured knowledge base (KB). In our work we are interested in the combination of text-based and structured resources for question answering, particularly articles that contain both tables and text. This is a natural next step for question answering on tables, in that most tables are embedded in documents that discuss them, creating a challenge of determining whether the answer is in the text or the table (if anywhere). In addition, very often information presented in tables is compact and limited. The associated text provides a rich context that can be used to enhance the representation of the table for more robust question answering. 

Consider the example in \cite{PasupatLiang15} of the table of summer Olympic games shown in Figure \ref{fig: qa_olympiad_example}. This is one of four tables in the associated Wikipedia article. The heading of the first column is ``Olympiad," but in the text they are most often referred to as ``games". The heading ``games'' is used in a different table for a column related to the number of Olympiads that a country has participated in. Linking the phrase "The United States hosted the games four times (in 1904, 1932, 1984 and 1996)" to the related cells in the table provides a mechanism to interpret that relation for other countries. 


In order for question answering to work effectively on tables, it is important to start with a good table representation. A table is an example of text represented in a structured way. Text in tables have special relations, such as relations between cells and corresponding row and column headers, or nearby table cells.  %On one hand, using some standard language representation  architectures,  such  as  BERT  \cite{devlin2018bert},  gives  an  advantage of good initialized pretrained representations for text contained in cells of the table. %Explicit modeling on table structure can benefit learning dependencies across table cells.
Standard contextualized representations of language, such as BERT \cite{devlin2018bert}, are trained on sentences. When applied to text in a table, it is not clear whether a ``sentence" should be a row, a column or a cell. While all choices provide some context, they fall short because table context is two-dimensional, not linear.
In this work, we extend the BERT architecture in order to allow to account for inter-cell relations. In addition, we  focus our work on learning a better table representation from the associated text discussion to provide a more robust table representation. We evaluate our approach on the Natural Questions corpus \cite{47761} that consist of real anonymized queries issued to the Google search engine and corresponding Wikipedia articles, that most of the time contain both tables and text. 

\begin{figure*}[t]
%   \vspace{-1cm}
    \begin{center}
    \includegraphics[width=1\textwidth]{example3.png}    
    \end{center}
    \caption{Fragments of text and a table from the Wikipedia article on Summer Olympics Games with correspondences underlined.}
    \label{fig: qa_olympiad_example}
\end{figure*}


Overall, the main contributions of our work are two-fold. First, we generalize RoBERTa \cite{liu2019roberta} to capture table representations, motivated by Graph Neural Networks with a transformer introduced by Shaw \textit{et al.}\   \cite{shaw2018self} that generalized a transformer for multiple types of relations used for relative position encoding. We pretrain new relations using a large table corpus extracted from Wikipedia \cite{bhagavatula2013methods}. Secondly, we introduce a novel mechanism of updating table representations based on text surrounding the table. We report our results on the Natural Questions (NQ) corpus, improving the baseline in Alberti \textit{et al.}\ \cite{alberti2019bert} on question answering on tables.


